Tensor Network Space-Time Spectral Collocation Method for Solving the Nonlinear Convection Diffusion Equation

Spectral methods provide highly accurate numerical solutions for partial differential equations, exhibiting exponential convergence with the number of spectral nodes. Traditionally, in addressing time-dependent nonlinear problems, attention has been on low-order finite difference schemes for time discretization and spectral element schemes for spatial variables. However, our recent developments have resulted in the application of spectral methods to both space and time variables, preserving spectral convergence in both domains. Leveraging Tensor Train techniques, our approach tackles the curse of dimensionality inherent in space-time methods. Here, we extend this methodology to the nonlinear time-dependent convection-diffusion equation. Our discretization scheme exhibits a low-rank structure, facilitating translation to tensor-train (TT) format. Nevertheless, controlling the TT-rank across Newton's iterations, needed to deal with the nonlinearity, poses a challenge, leading us to devise the "Step Truncation TT-Newton" method. We demonstrate the exponential convergence of our methods through various benchmark examples. Importantly, our scheme offers significantly reduced memory requirement compared to the full-grid scheme.

==> sec2_model.tex <==
\section{Mathematical Model and Numerical Discretization \ductodo{Dibyendu}}
\label{Model:problem}

\subsection{Nonlinear Convection-Diffusion-Reaction (NCDR) Equation }
\label{eq:model:problem}

We are interested in the following NCDR problem: Find
$u(t,\mathbf{x})$ such that,
\begin{align}
    \frac{\partial u}{\partial t}- a(u) \Delta u + \bold{b}(u)\cdot \nabla u + c(u)u&= F(u)  \quad \forall (t,\bold{x}) \in [0,T] \times \Omega \label{Model:Eqn1}\\
    u(t,\bold{x})&=g(t,\bold{x}) \quad \text{on}  \quad [0,T]\times \partial \Omega \label{Model:Eqn2}\\
    u(0,\bold{x})&= h(\bold{x}) \quad \text{on} \; \label{Model:Eqn3}\Omega,
\end{align}
\if
where $a(u)$, $b(u)$, and $f(u)$ are nonlinear diffusion, convection coefficients and nonlinear force function respectively. Further $\Omega \subset \mathbb{R}^{3}$ is a separable domain such as a $3$ dimensional flat torus or a Cartesian product of $3$ real intervals $\Omega_i=[a_i,b_i]$
\begin{equation*}
    \Omega= \otimes_{i=1}^{3} \Omega_i.
\end{equation*}
We summarize the the notation that will be necessary in the description of the methods. Fix a positive integer $N$. Let $x_1,x_2,\ldots,x_{N+1}$ denote the Legendre \ductodo{Change to Chebyshev} Gauss-Lobatto nodes with $x_1=a_i$, $x_{N+1}=b_i$, and $x_j$ are zeros of $\frac{dL_N}{dx}$ for $2 \leq j \leq N$. The Legendre Gauss nodes along the time direction is denoted by $\{ t_k\}$. For $0 \leq j \leq N$, let $l_j$ be the Lagrange interpolant, a polynomial of degree $N$, of $\{x_j\}$ so that $l_j(x_k)= \delta_{jk}$.  Recall that the for $N$, the Legendre derivative matrix $D \in \mathbb{R}^{(N+1) \times (N+1)}$ has entries 
\begin{equation*}
    D_{jk}=\frac{d l_k (x_j)}{d x} \quad \forall \;  0 \leq j,k \leq N.
\end{equation*}
An important property is that for a polynomial $\mathcal{P}_m(x)$ with $0 \leq m \leq 2N-1$,
\begin{equation}
\int_{-1}^{1} \mathcal{P}_m(x) dx= \sum_{k=1}^{N+1} \mathcal{P}_m(x_k) \rho_k,
\end{equation}
where $\{ \rho_k\}$ is the set of weights associated with Legendre Gauss-Lobatto quadrature. If $v$ is an analytic function, then it is known that 
\begin{equation}
   \Big \vert \int_{-1}^{1} v(x) dx-\sum_{j=1}^{N+1} v(x_j) \rho_j \big \vert \leq C~e^{-cN},
\end{equation}
where $c$ or $C$ are positive generic constants whose values may be different at different occurrence, and are independent of $N$. Let $W_h$ be the $(N+1) \times (N+1)$ diagonal matrix whose diagonal entries are $\{ \rho_k\}$. For any continuous function $v$ on $\Omega$, define the discrete norm 
\begin{equation*}
    \parallel v \parallel_N := \Big( \sum_{j,k=1}^{N+1} \rho_j \rho_k \vert v(t_k,x_j) \vert^2 \Big)^{1/2}.
\end{equation*}
For an integer $N \geq 2$, we first recall the space-time Legendre spectral collocation method. We first write the discrete function at $t=t_n$, 
\begin{equation*}
    u_k(t)= \sum_{q=1}^{N+1} \alpha_{qk} L_q(t). \quad 0 \leq k \leq N.
\end{equation*}
It is not difficult to show that 
\begin{equation*}
    \alpha_{qk}= 
    \begin{cases}
    & \frac{1}{(N+1) L_N(t_k) }, \quad q= N; \\
    & \frac{2q+1 L_q(t_k)}{N(N+1) L_N^2(t_k)}, \quad 0 \leq q \leq N.
    \end{cases}
\end{equation*}
For any real time $t$, define 
\begin{equation*}
    \bu_h(t)= \begin{bmatrix}
    u(x_1,t) \\
    \vdots \\
    u(x_{N+1,t})
    \end{bmatrix},
   \quad  \bff_h(t)= \begin{bmatrix}
    f(u(x_1,t)) \\
    \vdots \\
    f(u(x_{N+1,t}))
    \end{bmatrix}.
\end{equation*}
A semi-discrete approximation of \eqref{Model:Eqn1} is 
\begin{equation}
    \frac{d \bu_h(t)}{dt}=\diag(a(\bu_h(t))) \Delta \bu_h(t)-\diag(\bb(\bu_h(t))) \nabla \bu_h(t) + \bff_h(t).  
\end{equation}
For the time-discretization, the popular, technique is finite difference. Below, we summarize both the time-stepping method and space-time method.
\fi
where $a(u)$, $\Vec{b}(u)$, and $c(u)$ are
the non-linear: diffusion, convection and reaction coefficients, respectively, while $F(u)$ is the non-linear force function, and below we will denote $f(u):=-c(u)u+F(u)$.
%%
Furthermore, $\Omega\subset\mathbb{R}^3$ be a three dimensional, open
parallelepipied domain with boundary $\partial \Omega$; $h(\bold{x})$
is the initial condition, (IC), and $g(t,\bold{x})$ are the boundary
conditions (BC).
%%
Here we denote the 3D vectors, such as, $\Vec{x}=(x,y,z)$, and
matrices, in bold font.

\subsection{Chebyshev collocation method \ductodo{duc: update the references}}
\label{sec:spacetimeapproach}

%% \subsubsection{Space-time spectral collocation method}
%%
\if
The CDR equation contains both space and time variables and the
associated differential operators.
Here, we consider the discretization in space and time simultaneously
and thus we will work with a \emph{space-time} operator scheme that
simultaneously works in both the spatial and temporal dimensions.
Using a space-time approach simplifies the formulation and
implementation of the numerical algorithm.
The space-time approach is accurate for phenomena with rapidly
changing dynamics where the interaction between spatial and temporal
variations is significant \cite{marion2013classical}.
A traditional disadvantage of the space-time approach is the extension
of the number of dimensions, which consequently increases the
computational cost and memory requirements due to the curse of
dimensionality.
However, we will demonstrate that using tensor network machinery will
overcome this problem.
Classical numerical methods to solve the CDR equation are finite
difference approaches \cite{leveque2007finite} and spectral
collocation methods \cite{funaro1997spectral}.
\fi

%% Here we utilize spectral collocation discretization for the space-time
%% approach.\cite{khoromskij2011d}
%%
We expand the approximate solution of the CDR equation on the set of
orthogonal Chebyshev polynomials $T_k(x)$ = cos(k*arcos(x)) as global
basis functions.
%%
Then, we enforce the CDR equation at a discrete set of points within
the domain, known as \emph{collocation points}, leading to a system of
equations for the unknown expansion coefficients that we can solve.
%%
The collocation points of the Chebyshev grid are defined as in
\cite{hussaini1989spectral}, and form the so-called
\emph{collocation grid}, cf.~\cite{funaro1997spectral}.
%%
To this end, we need expressions for the derivatives of the
approximate solution on the Chebyshev grid.
%%
The derivative expansion coefficients with respect to the same set of
Chebyshev polynomials are determined by multiplying the matrix
representation of the partial differential operators and the expansion
coefficients of the numerical solution.
%%
In the rest of this section, we construct the time derivative,
${\partial}\slash{\partial t}$, the gradient, $\nabla$, and the
Laplacian, $\Delta $.
%%
To simplify such matrix representations, we modify the Chebyshev
polynomials (following Ref.~\cite{funaro1997spectral}), and construct
a new set of $N$-th degree polynomials $l_j$, $0\leq j\leq N$, with
respect to the collocation points, $x_i$, $0\leq i\leq N$, that
satisfy:
%%
\begin{equation}
  l_j(x_i) = 
  \left \{
  \begin{aligned}
    & 1 \qquad \text{if } \ i=j, \\
    & 0 \qquad \text{if } \ i \neq j.
  \end{aligned}
  \right.
\end{equation}
%%
Using the new polynomials $l_j$, the discrete CDR solution becomes,  
\begin{equation}
\label{Int_legen}
    u_h(x):= \sum_{j=0}^N u(x_j) l_j(x).
\end{equation}

We construct all the spatial partial differential operators using
the matrix representation of the single, one-dimensional derivative,
$\bold{S}_x$, which reads as
\begin{equation}
  \left(\frac{\partial}{\partial x}\right)_{ij} \rightarrow 
  (\bold{S}_x)_{i j}:= \frac{d}{dx}l_j(x)\Big|_{x_i}.
  \label{time_derivative}
\end{equation}
%%
The size of the matrix $\bold{S}_x$ is $(N+1) \times (N+1)$.
%%
We obtain the second order derivative matrix, $\bold{S}_{xx}$, by
matrix multiplication of the first order derivatives as,
%%
\begin{equation}
  (\bold{S}_{xx})_{ij} = \sum_{s=0}^{N} (\bold{S}_x)_{is} (\bold{S}_x)_{sj}.
\end{equation}
For completeness, we refer to \cite{funaro1997spectral} for the
derivation of this expression.

\if
As a numerical method for PDEs, the Chebyshev collocation method
demonstrates \cite{funaro1997spectral}:
%%
$(i)$ High accuracy, based on its exponential convergence rate with the
number of degrees of freedom;
%%
$(ii)$ Accuracy for capturing complex variations of the solution, based
on the use of smooth basis functions;
%%
$(iii)$ A global approximation, since each basis function affects the
entire domain and is suitable for problems with non-local
dependencies.
%%
Chebyshev collocation method requires regular grids, that is, it works
mainly on Cartesian grids that are tensor products of 1-D domain
partitions, which is suitable to our tensor network formats.
\fi

\subsubsection{Matrix form of the discrete NCDR equation}

First, we introduce the \emph{space-time} matrix operators: $\frac{\partial}{\partial t}
\rightarrow$ $\bold{A}_{t}$; $ \Delta $
$\rightarrow$ $\bold{A}_{D}$; $\nabla $
$\rightarrow$ $\bold{A}_{C} = [\bold{A}_{C}^x,\bold{A}_{C}^y,\bold{A}_{C}^z]$; and 
$f(u)$ $\rightarrow$ $\bold{F}(\bold{U})$ ; respectively.
%%
Upon employing these matrices, Eq.(\ref{Model:Eqn1}) results in
the following nonlinear system,
\begin{equation}
  \bold{A}_{t}\bold{U}+ a(\bold{U})\bold{A}_{D}\bold{U}+(\bold{b}(\bold{U})\cdot\bold{A}_{C})\bold{U}) = \bold{F}(\bold{U}),
  \label{Mat_System}
\end{equation}
where $\bold{U}$ is the vector corresponding to the
solution.
%%
The matrices $\bold{A}_{t}$, $\bold{A}_{D}$, $\bold{A}_{C}$, and
are of size $(N+1)^4 \times (N+1)^4$ for $N^{th}$ order
spectral collocation method, while $\bold{U}$, $\bold{F}$ are column
vectors of size $(N+1)^4 \times 1$.
\begin{equation}
\begin{split}
    \bA_t&:= \bS_t \otimes \I_{\text{space}}, \\
    \bA_D &:= \I_t \otimes \I_z \otimes \I_y \otimes \bS_{xx} +\I_t \otimes \I_z \otimes \bS_{yy} \otimes \I_xx + \I_t \otimes \bS_{zz} \otimes \I_{yy} \otimes \I_{xx}, \\
    \bold{b}(\bold{U})\cdot\bA_C &:= \textbf{diag}(b^x(\bold{U})) (\I_t \otimes \I_z \otimes \I_y \otimes \bS_{x})+\textbf{diag}(b^y(\bold{U})) (\I_t \otimes \I_z \otimes \bS_y \otimes \I_{x}) \\
     & \quad +\textbf{diag}(b^z(\bold{U})) (\I_t \otimes \bS_z \otimes \I_y \otimes \I_{x})\\
     F(\bold{U})&:= \textbf{diag}(f(\bold{U})) (\I_t \otimes \I_z \otimes \I_y \otimes \I_{x})
    \end{split}
\end{equation}


% \if
% \paragraph{Time-stepping method}
% In this approach, we discretize the time derivative part by using finite difference and space derivative by spectral collocation methods. The discrete scheme is stated as follows
% \begin{equation}
% \label{FD_SC_ST}
%     \begin{split}
%         \frac{\bu_h(t_{n})-\bu_h(t_{n-1})}{\Delta t}&= \diag(a(\bu_h(t_{n}))) \Delta \bu_h(t_{n})-\diag(\bb(\bu_h(t_{n}))) \nabla \bu_h(t_n) + \bff_h(t_n) \\
%         \bu_h(t_n) &=g(t_n) \quad \text{on} \; \partial \Omega \\
%         \bu_h(t_0) &= \bu_0 \; \text{on} \; \Omega. 
%     \end{split}
% \end{equation}
% By following \cite{}, we rewrite \eqref{FD_SC_ST} as follows
% \begin{equation}
% \label{Non_System}
%      (1/\Delta t)\bI_{\text{space}}U^n-\diag(a(\bold{U}^n)) \Delta U^n+ \diag(\bb(\bold{U}^n))  \nabla U^n-\bF( U^n)=(1/\Delta t)\bI_{\text{space}}U^{n-1},  
% \end{equation}
% where $\bF$ is the load vector. 
% \fi
\paragraph{How to deal with initial and boundary conditions}
To deal with the inhomogenous initial and boundary conditions in Eq.~\eqref{Model:Eqn2} and Eq.~\eqref{Model:Eqn3}, we choose to rewrite the Eq.~\eqref{Mat_System} as a nonlinear system of only interior nodes with the IC/BC incorporated in the term $\bold{F}^{bc}(\bold{U})$. This process is described in details in~\cite{adak2024tensor}. The nonlinear system for interior nodes becomes
\begin{equation}
  \bold{A}_{t}\bold{U}+ a(\bold{U})\bold{A}_{D}\bold{U}+(\bold{b}(\bold{U})\cdot\bold{A}_{C})\bold{U}) = \bold{F}(\bold{U}) - \bold{F}^{bc}(\bold{U}),
  \label{Mat_int_System}
\end{equation}

The nonlinear system  \eqref{Mat_int_System} can be solved by employing Newton's method.


\paragraph{Newton's Methods:}

For better explanation, we would like to explore Newton's Methods for strong form of \eqref{Model:Eqn1} briefly. We first write $u$ as 
\begin{equation}
    u=u^0+\delta,
\end{equation}
where $u^0$ is some known approximation of $u$, and $\delta$ is a correction. This gives us
\begin{equation}
\label{Newton:1}
    \frac{\partial (u^0+\delta)}{\partial t}- a(u^0+\delta) \Delta (u^0+\delta) + \bold{b}(u^0+\delta)\cdot \nabla u -F(u^0+\delta)=0
\end{equation}
Now, we expand the nonlinear coefficients $a(u^0+\delta)$, $\bold{b}(u^0+\delta)$, and nonlinear force function $F(u^0+\delta)$ by using Taylor expansion such as follows.
\begin{equation}
\label{taylor_coefficient}
    \begin{split}
        a(u^0+\delta)&= a(u^0)+a'_u(u^0) \delta+ O(\delta^2);\\
        \bb(u^0+\delta)&= \bb(u^0)+\bb'_u(u^0) \delta+ O(\delta^2);\\
    F(u^0+\delta)&=F(u^0)+F'_u(u^0) \delta+ O(\delta^2).
    \end{split}
\end{equation}
By inserting \eqref{taylor_coefficient} into \eqref{Newton:1}, and neglecting terms involving $\delta^2$, $\delta \Delta \delta$, and $\delta \nabla \delta$, we deduce that
\begin{equation} 
\label{Newton:2}
\begin{split}
   & \frac{\partial \delta}{ \partial t}-a(u^0) \Delta \delta- a'_u(u^0) \Delta u^00 \delta + \bb'_u(u^0) \cdot \nabla u^0+\bb(u^0) \nabla \delta -\delta F'_u(u^0) \\
    &=F(u^0)- \Big( \frac{\partial u^0}{ \partial t}-a(u^0) \Delta u^0+ \bb(u^0) \cdot \nabla u^0 \Big ).
    \end{split}
\end{equation}
Further, we define 
\begin{equation}
\begin{split}
    J \delta &:= \frac{\partial \delta}{ \partial t}-a(u^0) \Delta \delta- a'_u(u^0) \Delta u^0 \delta + \bb'_u(u^0) \cdot \nabla u^0+\bb(u^0) \nabla \delta -\delta F'_u(u^0), \\
    \text{Res} &= F(u^0)- \Big( \frac{\partial u^0}{ \partial t}-a(u^0) \Delta u^0+ \bb(u^0) \cdot \nabla u^0 \Big ),
    \end{split}
\end{equation}
and consequently, \eqref{Newton:2} can be written as, Find $\delta$ such that
\begin{equation}
\label{Newton:3}
    J \delta=\text{Res}.
\end{equation}
Once we have found $\delta$, the Newton  method is then to set $u^1=u^0+\delta$
and iterate, starting with the new solution guess $u^1$.
%
\paragraph{Spectral Collocation Approximation:}
Here, we assume that $u_h^0 \in V_h$ is an initial guess. The Spectral collocation approximation of \eqref{Newton:3} reads as follows: Find $\delta_h \in V_h$ such that
\begin{equation}
\label{Dis:system}
    J_h \delta_h =\text{Res}_h,
\end{equation}
where $J_h$, and $\text{Res}_h$ are the spectral approximation  of the operator $J$, and $\text{Res}$ respectively. 
 The new initial guess is defined as $u_h^{1}:= u_h^0+\delta_h$. Since $\delta_h, u_h^0 \in V_h$, we can write explicitly as below
\begin{equation}
\label{Discrete:Newton}
    \begin{split}
        \delta_h &:= \sum_{j=1}^{N+1} \delta_j l_j(x);\\
        u_h^0 &:= \sum_{j=1}^{N+1} U_j^0 l_j(x).
    \end{split}
\end{equation}
Inserting \eqref{Discrete:Newton} into \eqref{Newton:3}, we obtain a system of linear equation in $\delta_h$. The corresponding matrization of the residual operator is derived as follows.
\begin{equation}
\label{residual:1}
    \textbf{Res}(\bold{U}^0) := F(\bold{U}^0)- \Big ( \bA_t +\bA_D(\bold{U}^0) +\bA_C(\bold{U}^0)\Big)\bold{U}^0.
\end{equation}
\if
We will explore both techniques. In fixed-point technique, the nonlinear system \eqref{Non_System} can be reduces to linear system in the following way. Given $\bold{U}^{n-1}$, find $\bold{U}^n$  such that
\begin{equation}
\label{Non_System}
     (1/\Delta t)\bI_{\text{space}}U^n-\diag(a(\bold{U}^{n-1})) \Delta U^n+ \diag(b(\bold{U}^{n-1}))  \nabla U^n-\bG( U^{n-1})U^n=(1/\Delta t)\bI_{\text{space}}U^{n-1},  
\end{equation}
where $\bG( U^{n-1})U^n$ is the linearization of the $\bF(U)$. The fixed-point has linear order of convergence, whereas Newton method has quadratic order of convergence. 

%Here, we will utilize the Newton method to solve \eqref{Mat_System}.

The residual vector corresponding to \eqref{Mat_System} can be written as follows,
\begin{equation}
    \textbf{Res}(\boldsymbol{U^{(n)}}):= (1/\Delta t)\bI_{\text{space}}U^n-\diag(a(\bold{U}^n)) \Delta U^n+ \diag(b(\bold{U}^n))  \nabla U^n-\bF( U^n)-(1/\Delta t)\bI_{\text{space}}U^{n-1}.
\end{equation}
Here, the Jacobian matrix is defined as follows
\begin{equation}
\begin{split}
    \J &:= (1/\Delta t) \bI_{\text{space}}-\diag(a(\bold{U}^n)) \Delta - \diag(a'(\bold{U}^{n})\Delta U^n )+ \diag(b(\bold{U}^n)) \nabla \\
    & \qquad + \diag(b'(\bold{U}^n) \nabla U^n )-\diag(\bF'(U^n)).  
    \end{split}
\end{equation}
By employing the $\textbf{Res}$, and $\J$, we compute the correction at each iteration in the nonlinear loop. 

\paragraph{Matrization of the convective term}
Let us consider the vector valued convective term $$\bb(\bold{U})= [b_1(\bold{U}) b_2(\bold{U}) b_3(\bold{U})]^{T}.$$
In particular, 
\begin{equation}
\begin{split}
    \bb(\bold{U}) \nabla \bold{U} &= b_1(\bold{U}) \frac{\partial}{\partial x} \bold{U}+b_2(\bold{U}) \frac{\partial}{\partial y} \bold{U}+b_3(\bold{U}) \frac{\partial}{\partial z} \bold{U}\\
    & =\diag(b_1(\bold{U})) (\I_t \otimes \I_z \otimes \I_y \otimes \bS_x) \bold{U}+ \diag(b_2(\bold{U})) (\I_t \otimes \I_z \otimes \bS_y \otimes \I_x) \bold{U} \\
    & \quad + \diag(b_3(\bold{U})) (\I_t \otimes \bS_z \otimes \I_y \otimes \I_x) \bold{U}.
    \end{split}
\end{equation}




\subsection{Spectral scheme for the Space-Time operator} 

In this section, we would like to display the Spectral collocation scheme for the nonlinear heat equation (\eqref{Model:Eqn1}-\eqref{Model:Eqn3}). We first construct the residual vector as follows

\begin{equation}
\label{Eqn:Nonlinear}
   [ \bS_t \otimes \I_{\text{space}}-\text{diag}(\boldsymbol{a(U)}) \Delta]\boldsymbol{U} -\text{diag}(\boldsymbol{F(U)}) (\I_t \otimes \I_x) =0,
\end{equation}
where the discretization for the Laplace operator is defined as

\begin{equation}
\label{Eqn:Delta}
    \Delta= \I_t \otimes \bS_{xx} \otimes \I_y \otimes \I_z+\I_t \otimes \I_x \otimes \bS_{yy} \otimes \I_z + \I_t \otimes \I_x \otimes \I_y \otimes \bS_{zz}.
\end{equation}
The system of nonlinear equation can be solved by employing Picards' Iteration technique or Newton's methods. Further, we highlight that the order of convergence for the Picards' Iteration is linear whereas for Newton, the order of convergence is quadratic. For better explanation, we discussed the scheme in details.  
\paragraph{Picard's Iteration}
In \eqref{Eqn:Nonlinear}, the nonlinear diffusion coefficients and the nonlinear force function satisfy the Lipschitz's continuity condition which guarantee the well-posedness of the scheme. In particular, we choose the nonlinear diffusion coefficients $a(u):=u^2$, and the force function $f(u):= u^3$. With these choice, we linearize the nonlinear system of equation \eqref{Model:Eqn1}-\eqref{Model:Eqn3} as follows 
\begin{equation}
    [ \bS_t \otimes \I_{\text{space}}-\text{diag}((\boldsymbol{U^{(n)}})^2) \Delta -\text{diag}((\boldsymbol{U^{(n)})^2}) (\I_t \otimes \I_x)]\boldsymbol{{U}^{n+1} }=0 \quad \forall n=0,1,2\ldots N_{\text{Max}}.
\end{equation}
%
\fi
We define the Jacobian Matrix $\J$ corresponding to the residual vector \eqref{residual:1} as 
\begin{equation}
    (\J)_{ij}:= \frac{\partial \textbf{Res}_i(\boldsymbol{U^{(0)}})}{\partial \boldsymbol{U^{(0)}_j} }.
\end{equation}
%where
%\begin{equation}
%    \textbf{Res}_i(\boldsymbol{U^{(n)}}):= \Big [ \bS_t \otimes \I_{\text{space}}-\text{diag}((\boldsymbol{U^{(n)}})^2) \Delta -\text{diag}((\boldsymbol{U^{(n)})^2}) (\I_t \otimes \I_x) \Big ]\boldsymbol{{U}^{n+1}_i }. 
%\end{equation}
%Consequently, 
The Jacobian matrix is derived as follows
\begin{equation}
\begin{split}
    \J  = \Big [ \bS_t \otimes \I_{\text{space}}- \textbf{diag}(a'_u(\boldsymbol{U^{(0)}})) \textbf{diag} (\Delta \boldsymbol{{U}^{0} })-&\text{diag}(a(\boldsymbol{U^{(0)}})) \Delta \\
    &- \text{diag}(F_u'(\boldsymbol{U^{(0)})}) (\I_t \otimes \I_{\text{space}})\Big ].
    \end{split}
\end{equation}
\eqref{Dis:system} can be written in matrix form as
\begin{equation}
\J \boldsymbol{\delta} =\textbf{Res}.
\end{equation}
The new initial guess is modified as 
\begin{equation}
\bold{U}^1=\bold{U}^0+\boldsymbol{\delta},
\end{equation}
where
\begin{equation*}
   \bold{U}^1 = \begin{bmatrix}
    U_1^1 \\
    \vdots \\
    U_{N+1}^1 
    \end{bmatrix}_{N+1 \times 1},
   \quad  \bold{U}^0 = \begin{bmatrix}
    U_1^0 \\
    \vdots \\
    U_{N+1}^0 
    \end{bmatrix}_{N+1 \times 1},
    \quad  \boldsymbol{\delta} = \begin{bmatrix}
    \delta_1 \\
    \vdots \\
    \delta_{N+1} 
    \end{bmatrix}_{N+1 \times 1}.
\end{equation*}


